VeriEQL: Bounded Equivalence Verification for Complex SQL Queries with Integrity Constraints

The task of SQL query equivalence checking is important in various real-world applications (including query rewriting and automated grading) that involve complex queries with integrity constraints; yet, state-of-the-art techniques are very limited in their capability of reasoning about complex features (e.g., those that involve sorting, case statement, rich integrity constraints, etc.) in real-life queries. To the best of our knowledge, we propose the first SMT-based approach and its implementation, VeriEQL, capable of proving and disproving bounded equivalence of complex SQL queries. VeriEQL is based on a new logical encoding that models query semantics over symbolic tuples using the theory of integers with uninterpreted functions. It is simple yet highly practical -- our comprehensive evaluation on over 20,000 benchmarks shows that VeriEQL outperforms all state-of-the-art techniques by more than one order of magnitude in terms of the number of benchmarks that can be proved or disproved. VeriEQL can also generate counterexamples that facilitate many downstream tasks (such as finding serious bugs in systems like MySQL and Apache Calcite).

==> fig-example-emp-dept.tex <==
\begin{figure}[H]
\scriptsize
\begin{subfigure}[b]{0.3\textwidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
eid & ename & did \\
\hline
1 & A & 11 \\
\hline
2 & B & 12 \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{\texttt{EMP}}
\end{subfigure}
~
\begin{subfigure}[b]{0.3\textwidth}
\centering
\begin{tabular}{|c|c|}
\hline
id & dname \\
\hline
10 & C \\
\hline
11 & D \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{\texttt{DEPT}}
\end{subfigure}
\end{figure}


==> fig-example-joins-only.tex <==
\begin{figure}[H]
\scriptsize
\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
eid & ename & did & id & dname \\
\hline
1 & A & 11 & 11 & D \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{$\texttt{EMP} \ijoin_{\texttt{did=id}} \texttt{DEPT}$}
\end{subfigure}
~
\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
eid & ename & did & id & dname \\
\hline
1 & A & 11 & 11 & D \\
\hline
2 & B & 12 & \sqlnull & \sqlnull \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{$\texttt{EMP} \ljoin_{\texttt{did=id}} \texttt{DEPT}$}
\end{subfigure}
~
\begin{subfigure}[b]{0.35\textwidth}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
eid & ename & did & id & dname \\
\hline
\sqlnull & \sqlnull & \sqlnull & 10 & C \\
\hline
1 & A & 11 & 11 & D \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{$\texttt{EMP} \rjoin_{\texttt{did=id}} \texttt{DEPT}$}
\end{subfigure}

\vspace{10pt}

\begin{subfigure}[b]{0.35\textwidth}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
eid & ename & did & id & dname \\
\hline
1 & A & 11 & 11 & D \\
\hline
2 & B & 12 & \sqlnull & \sqlnull \\
\hline
\sqlnull & \sqlnull & \sqlnull & 10 & C \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{$\texttt{EMP} \fjoin_{\texttt{did=id}} \texttt{DEPT}$}
\end{subfigure}
~
\begin{subfigure}[b]{0.35\textwidth}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
eid & ename & did & id & dname \\
\hline
1 & A & 11 & 10 & C \\
\hline
1 & A & 11 & 11 & D \\
\hline
2 & B & 12 & 10 & C \\
\hline
2 & B & 12 & 11 & D \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{$\texttt{EMP} \times \texttt{DEPT}$}
\end{subfigure}

\end{figure}


==> fig-example-mysql-bug-simplified.tex <==
% simplified version
% \pztodo{We found a bug in MySQL that leads to incorrect query results.  Table \ref{tab:mysql-example-queries} shows a simplified example that epitomizes the 2 $\leetcode$ benchmarks with spurious counterexamples while can reproduce the bug.  Noticeably, $Q_1$ and $Q_2$ are semantically different and different only in one spot that $Q_1$ uses \sqljoin whereas $Q_2$ uses \sqlleftjoin.  \tool, naturally, produces a counterexample as shown in Figure \todo{?} for this query pair that would theoretically be able to demonstrate their non-equivalence, but, as we checked their results by running them on a MySQL server, both of them output an empty set.  However, $A$ \sqlleftjoin $B$ will necessarily retain all records in table $A$ in the output, while all columns in table $B$ will be \sqlnull after joining because the \sqlon clause predicate will be always evaluated to false with the DB provided.  Also, the \sqlwhere predicate will always be evaluated to true since T2.ID (i.e., B.ID, which is 3) will not be in an empty set.  Therefore, the result of the subquery $T$ in $Q_2$ should be as shown in Figure \todo{?}.  We confirmed that the output of the subquery $T$ on MySQL per se conforms to what is expected.  But, given that the main query of $Q_2$ performs nothing additionally but just a projection over the subquery $T$, the output of $Q_2$ should be the same as its subquery $T$.  Therefore, we believe it is incorrect that $Q_2$ running on such a counterexample DB would produce an empty set, instead of the same result as $T$.  As this behavior was reproducible on MySQL's latest release version, 8.0.32, we opened a bug report for this issue, which was then verified the MySQL Verification Team.}


\begin{table}[H]
\scriptsize
\begin{tabular}{|l|l|}
\hline
$Q_1$ & \begin{tabular}[c]{@{}l@{}}

\sqlselectcolor T2.ID \sqlascolor ID \\
\sqlfromcolor A \sqlascolor T1 \sqljoincolor B \sqlascolor T2 \\ 
\sqloncolor T1.ID = T2.ID \\
\sqlwherecolor T1.ID \sqlnotcolor \sqlincolor (\sqlselectcolor ID \sqlfromcolor A \sqlwherecolor ID = 3)

\end{tabular}         \\ \hline
$Q_2$  & \begin{tabular}[c]{@{}l@{}}

\sqlselectcolor ID \sqlfromcolor ( \\
\hspace{1em}  \sqlselectcolor T2.ID \sqlascolor ID \\
\hspace{1em}  \sqlfromcolor A \sqlascolor T1 \sqlleftjoincolor B \sqlascolor T2 \\ 
\hspace{1em}  \sqloncolor T1.ID = T2.ID \\ 
\hspace{1em}  \sqlwherecolor T2.ID \sqlnotcolor \sqlincolor (\sqlselectcolor ID \sqlfromcolor A \sqlwherecolor ID = 3) \\ 
) T

\end{tabular} \\ \hline
\end{tabular}
\caption{MySQL Example}
\vspace{-20pt}
\label{tab:mysql-example-queries}
\end{table}

\begin{figure}[H]
\scriptsize

\begin{subfigure}[b]{0.48\textwidth}
\begin{tabular}{|l|}
\hline
ID \\ \hline
2  \\ \hline
\end{tabular}
\caption{MySQL Example: Counterexample Table A}
\label{tab:mysql-example-counterexample-table-a}
\end{subfigure}


\begin{subfigure}[b]{0.48\textwidth}
\begin{tabular}{|l|}
\hline
ID \\ \hline
3  \\ \hline
\end{tabular}
\caption{MySQL Example: Counterexample Table B}
\label{tab:mysql-example-counterexample-table-b}
\end{subfigure}

\begin{subfigure}[b]{0.48\textwidth}
\begin{tabular}{|l|}
\hline
ID \\ \hline
\sqlnull  \\ \hline
\end{tabular}
\caption{MySQL Example: $Q_2$ Subquery $T$ Output}
\vspace{-20pt}
\label{tab:mysql-example-counterexample-q2-output}
\end{subfigure}


\end{figure}


==> fig-motivating-example.tex <==
\begin{table}[H]
\scriptsize
\begin{tabular}{|l|l|l|}
\hline
$\schema$ & \begin{tabular}[c]{@{}l@{}l@{}}

\{A: \{id: Integer\}, B: \{uid: Integer\} \}

\end{tabular}        
& \begin{tabular}[c]{@{}l@{}l@{}}

$\formula_\schema = \neg \del(t_1) \land \neg \del(t_2) \land \neg \del(t_3) \land \neg \del(t_4)$

\end{tabular}         \\ \hline

$\constraint$ & \begin{tabular}[c]{@{}l@{}l@{}}

PRIMARY KEY (A.id); \\
PRIMARY KEY (B.uid); 

\end{tabular}   
& \begin{tabular}[c]{@{}l@{}l@{}}

% \begin{align}
%     \formula_\constraint = t_1.id \neq \nullv \land t_2.id \neq \nullv \land t_1.id \neq t_2.id \land
% \end{align}

$ \formula_\constraint = t_1.id \neq \nullv \land t_2.id \neq \nullv \land t_1.id \neq t_2.id \land $ \\
$\land_{t \in [t_1, t_2]} -2^{31} \leq t.id \leq 2^{31}-1 \land \ldots$ \\
% $t_3.uid \neq \nullv \land t_4.uid \neq \nullv \land t_3.uid \neq t_4.uid$ \\
% $\land_{t \in [t_3, t_4]} -2^{31} \leq t.uid \leq 2^{31}-1$ 

\end{tabular}         \\ \hline

$\query_1$ & \begin{tabular}[c]{@{}l@{}l@{}}

\sqlselectcolor T2.uid \sqlascolor id \\
\sqlfromcolor A \sqlascolor T1 \sqljoincolor B \sqlascolor T2 \\
\hspace{1em}  \sqloncolor T1.id = T2.uid \\
\sqlwherecolor T1.id \sqlnotcolor \sqlincolor ( \\
\hspace{3em}  \sqlselectcolor id \sqlfromcolor A \sqlwherecolor id = 3 \\
\hspace{2em}  )

\end{tabular}      
& \begin{tabular}[c]{@{}l@{}l@{}}

\\
$\formula_{\rename} = t5 = t1 \land t6 = t2 \land t7 = t3 \land t8 = t4$ \\
$\formula_{\ijoin_\phi} = \land_{i \in [5,6]} \land_{j \in [7,8]} \neg \del(t_i) \land \neg \del(t_j) \to \neg \del(t_{i,j}) \land \ldots \land \del(t_i) \lor \del(t_j) \to \del(t_{i,j})$ \\
$\formula_{Q_{s}} = \land_{(t, t') \in [(t1, t9), (t2, t10)]} \neg \del(t) \land (t.id = 3) = \top \to  t' = t \land \del(t) \lor (t.id = 3) \neq \top \to \del(t')$

\end{tabular}         \\ \hline

$\query_2$  & \begin{tabular}[c]{@{}l@{}l@{}}

\sqlselectcolor id \sqlfromcolor ( \\
\hspace{1em}  \sqlselectcolor T2.uid \sqlascolor id \\
\hspace{1em}  \sqlfromcolor A \sqlascolor T1 \sqlleftjoincolor B \sqlascolor T2 \\
\hspace{1em}  \sqloncolor T1.id = T2.uid \\ 
\hspace{1em}  \sqlwherecolor T2.uid \sqlnotcolor \sqlincolor (\sqlselectcolor id \sqlfromcolor A \sqlwherecolor id = 3) \\ 
) T

\end{tabular} 
& \begin{tabular}[c]{@{}l@{}l@{}}

-

\end{tabular}         \\ \hline

\end{tabular}
\caption{A simplified motivating example.}
\vspace{-20pt}
\label{fig:motivating-example}
\end{table}

==> limit.tex <==
\section{Limitation} \label{sec:limit}


